Unsupervised Graph Spectral Feature Denoising for Crop Yield Prediction

Prediction of annual crop yields at a county granularity is important for national food production and price stability. In this paper, towards the goal of better crop yield prediction, leveraging recent graph signal processing (GSP) tools to exploit spatial correlation among neighboring counties, we denoise relevant features via graph spectral filtering that are inputs to a deep learning prediction model. Specifically, we first construct a combinatorial graph with edge weights that encode county-to-county similarities in soil and location features via metric learning. We then denoise features via a maximum a posteriori (MAP) formulation with a graph Laplacian regularizer (GLR). We focus on the challenge to estimate the crucial weight parameter $\mu$, trading off the fidelity term and GLR, that is a function of noise variance in an unsupervised manner. We first estimate noise variance directly from noise-corrupted graph signals using a graph clique detection (GCD) procedure that discovers locally constant regions. We then compute an optimal $\mu$ minimizing an approximate mean square error function via bias-variance analysis. Experimental results from collected USDA data show that using denoised features as input, performance of a crop yield prediction model can be improved noticeably.

==> journal/defs.tex <==
\def\0{{\mathbf 0}}
\def\1{{\mathbf 1}}

\def\a{{\mathbf a}}
\def\b{{\mathbf b}}
\def\c{{\mathbf c}}
\def\d{{\mathbf d}}
\def\e{{\mathbf e}}
\def\f{{\mathbf f}}
\def\g{{\mathbf g}}
\def\h{{\mathbf h}}
\def\i{{\mathbf i}}
\def\j{{\mathbf j}}
\def\k{{\mathbf k}}
\def\l{{\mathbf l}}
\def\m{{\mathbf m}}
\def\n{{\mathbf n}}
\def\o{{\mathbf o}}
\def\p{{\mathbf p}}
\def\q{{\mathbf q}}
\def\r{{\mathbf r}}
\def\s{{\mathbf s}}
\def\t{{\mathbf t}}
\def\u{{\mathbf u}}
\def\v{{\mathbf v}}
\def\w{{\mathbf w}}
\def\x{{\mathbf x}}
\def\y{{\mathbf y}}
\def\z{{\mathbf z}}

\def\A{{\mathbf A}}
\def\B{{\mathbf B}}
\def\C{{\mathbf C}}
\def\D{{\mathbf D}}
\def\E{{\mathbf E}}
\def\F{{\mathbf F}}
\def\G{{\mathbf G}}
\def\F{{\mathbf F}}
\def\H{{\mathbf H}}
\def\I{{\mathbf I}}
\def\J{{\mathbf J}}
\def\K{{\mathbf K}}
\def\L{{\mathbf L}}
\def\M{{\mathbf M}}
\def\N{{\mathbf N}}
\def\O{{\mathbf O}}
\def\P{{\mathbf P}}
\def\Q{{\mathbf Q}}
\def\R{{\mathbf R}}
\def\S{{\mathbf S}}
\def\T{{\mathbf T}}
\def\U{{\mathbf U}}
\def\V{{\mathbf V}}
\def\W{{\mathbf W}}
\def\X{{\mathbf X}}
\def\Y{{\mathbf Y}}
\def\Z{{\mathbf Z}}

\def\rE{{\text{E}}}
\def\rPr{{\text{Pr}}}
\def\Tr{{\text{Tr}}}
\def\vec{{\textrm{vec}}}
\def\ie{{\textit{i.e.}}}
\def\eg{{\textit{e.g.}}}
 

\def\cA{{\mathcal A}}
\def\cB{{\mathcal B}}
\def\cC{{\mathcal C}}
\def\cD{{\mathcal D}}
\def\cE{{\mathcal E}}
\def\cF{{\mathcal F}}
\def\cG{{\mathcal G}}
\def\cH{{\mathcal H}}
\def\cI{{\mathcal I}}
\def\cK{{\mathcal K}}
\def\cL{{\mathcal L}}
\def\cQ{{\mathcal Q}}
\def\cN{{\mathcal N}}
\def\cO{{\mathcal O}}
\def\cR{{\mathcal R}}
\def\cS{{\mathcal S}}
\def\cT{{\mathcal T}}
\def\cV{{\mathcal V}}
\def\cX{{\mathcal X}}
\def\cY{{\mathcal Y}}
\def\cZ{{\mathcal Z}}

\def\bphi{{\pmb{\phi}}}
\def\bpsi{{\pmb{\psi}}}
\def\bomega{{\pmb{\omega}}}
\def\balpha{{\boldsymbol \alpha}}
\def\bbeta{{\boldsymbol \beta}}
\def\bsigma{{\boldsymbol \sigma}}
\def\bvarphi{{\boldsymbol \varphi}}
\def\bsPhi{{\boldsymbol \Phi}}
\def\bsPsi{{\boldsymbol \Psi}}
\def\bsOmega{{\boldsymbol \Omega}}

==> journal/formulate.tex <==
\subsection{Graph Construction}

\red{In a similarity graph, each edge weight $w_{i,j}$ encode pairwise correlation / similarity between \textit{noiseless} signal samples $x_i$ and $x_j$.
Generally, there are two graph notions: deterministic and probabilistic.
In a deterministic interpretation, an edge weight $w_{i,j}$ encodes a function of the distance $d_{i,j}$ between nodes $i$ and $j$ on a smooth manifold that is inversely proportional to $d_{i,j}$.
In a probabilistic interpretation, an edge weight $w_{i,j}$ encodes the conditional correlation between samples $x_i$ and $x_j$ in a joint distribution like GMRF:
}

\begin{align}
\text{Corr}(x_i,x_j\,|\,\x_{-ij}) &= - \frac{Q_{ij}}{\sqrt{Q_{ii}Q_{jj}}}
\end{align}

In a practical scenario, one is provided only data; it is up to a practitioner to first construct an appropriate graph for subsequent graph-based processing, such as denoising, interpolation, etc.
Broadly speaking, there are two classes of graph learning approaches in the GSP literature: \textit{statistical} and \textit{deterministic}.
Statistical methods such as graphical lasso (GLASSO) \red{add ref} and its variants \red{add refs} assume multiple observations $\{\y_i\}_{i=1}^M$ generated from the same statistical model, such as \textit{Gaussian Markov Random Field} (GMRF) \red{add ref}, so that a reliable empirical covariance matrix $\C$ can be first calculated. 
A graph Laplacian matrix $\L$ close to $\C^{-1}$ is then computed with additional assumptions such as sparsity \red{add ref}, edge connectivity \red{add ref}, or edge weight signs \red{add refs}.

In contrast, deterministic methods do not assume multiple observations  $\{\y_i\}_{i=1}^M$, but assume \textit{relevant features} $\f_i \in \mathbb{R}^K$ per node $i$ are available, so that edge weight $w_{i,j} \propto d_{i,j}^{-1}$ between nodes $i$ and $j$ can be computed to be inversely proportional to \textit{feature distance} $d_{i,j}$.

\red{add graph metric learning discussion}.

We construct a similarity graph as follows. 



\subsection{Estimating Noise Variance}

In our feature denoising scenario, one must estimate the noise variance $\sigma^2$ directly from noisy feature (signal) $\y$, using which weight parameter $\mu$ in \eqref{eq:MAP} is computed.
We propose a noise estimation procedure called \textit{graph clique detection} (GCD) when a graph $\cG$ encoded with inter-node similarities is provided. 

We generalize from noise estimation in 2D images~\cite{wu2015}. 
First, we identify \textit{locally constant regions} (LCRs) $\cR_m$ where signal samples are expected to be similar, \ie, $x_i \approx x_j, \forall i,j \in \cR_m$. 
Then, we compute mean $\bar{x}_m = \frac{1}{|\cR_{m}|}\sum_{i \in \cR_m} x_i$ and variance $\sigma^2_m = \frac{1}{|\cR_{m}|} \sum_{i \in \cR_m} (x_i - \bar{x}_m)^2$ for $\cR_m$ accordingly.
Finally, we compute the global noise variance as the weighted average:
\begin{align}
\sigma^2 = \sum_m \frac{|\cR_m|}{\sum_k |\cR_k|}\sigma_m^2 .
\label{eq:noise_variance}
\end{align}

The crux thus resides in the identification of LCRs in a graph. 
We describe our proposal based on cliques. 
A \textit{clique} is a (sub-)graph where every node is connected with every other node in the (sub-)graph \red{add ref}. 
Thus, assuming edges represent pairwise similarities, a clique implies a node cluster with strong inter-node similarities, which we assume is roughly constant. 
Given an input graph $\cG$, we identify cliques in $\cG$ as follows. 


\subsubsection{$k$-hop Connected Graph}

\begin{figure}[t]
\centering
%\hspace{-30pt}
%\vspace{-10pt}
\subfloat[]{
\includegraphics[width=0.21\textwidth]{original1}
\label{fig:pcd-on}}
\hspace{-10pt}
%\subfloat[{}]{
%\includegraphics[width=0.33\textwidth]{2-hops1}
%\label{fig:pcd-off}}
%\hspace{-10pt}
\subfloat[{}]{
\includegraphics[width=0.24\textwidth]{cliques1}
\label{fig:pcd-off}}
%\hspace{-8pt}
\vspace{-0.05in}
\caption{(a) Example of a $10$-node graph, where edges with weights less than threshold $\hat{w}$ are colored in green; (b) The resulting k-hop connected graph (KCG) for $k=2$, after removing green edges and creating edges (colored in magenta) by connecting 2-hop neighbors. 
Two maximal cliques (out of 5) in KCG are highlighted.} %~\cite{bernardini1999}
\label{fig:cliques}
%\vspace{-14pt}
\end{figure}

We first sort $M = |\cE|$ edges in $\cG$ in weights from smallest to largest. 
For a given \textit{threshold weight} $\hat{w}$ and $k \in \mathbb{Z}^+$, we remove all edges $(i,j) \in \cE$ with weights $w_{i,j} < \hat{w}$ and construct a \textit{$k$-hop connected graph} (KCG)  $\cG^{(k)}$ with edges connecting nodes $i$ and $j$ that are $k$-hop neighbors in $\cG$.
If $\cG^{(k)}$ has at least $\hat{E}$ target edges, then it is a \textit{feasible} KCG with minimum connectivity 
\begin{align}
C(\cG^{(k)}) = \hat{w}^k.
\end{align}
$C(\cG^{(k)})$ is the weakest possible connection between two connected nodes in $\cG^{(k)}$ when interpreting edge weights $w_{i,j}$ as conditional probabilities, as done in \textit{Gaussian Markov Random Field} (GMRF)~\cite{rue2005}.  
Given $k$, we seek the \textit{largest} $\hat{w}$ while $\cG^{(k)}$ remains feasible via binary search among $M$ edges in complexity $\cO(\log M)$. 
We then increment $k$ and repeat the above procedure to find the largest $\hat{w}$, until we identify a maximal $\hat{w}^k$. 

See Fig.\;\ref{fig:cliques}(b) for an example of a KCG $\cG^{(2)}$ given original graph $\cG$ in Fig.\;\ref{fig:cliques}(a). 
We see, for example, that edge $(3,10)$ is removed from $\cG$, but edge $(4,10)$ is added in $\cG^{(2)}$ because nodes $4$ and $10$ are $2$-hop neighbors in $\cG$. 
The idea is to identify strongly similar pairs in original $\cG$ and connect them with explicit edges in $\cG^{(k)}$. 
Then the maximal cliques\footnote{A maximal clique is a clique that cannot be extended by including one more adjacent node. Hence, a maximal clique is not a sub-set of a larger clique in the graph.} are discovered using algorithm in \cite{cazals2008note}, as shown in Fig.\;\ref{fig:cliques}(b).
The cliques in the resulting graph $\cG^{(k)}$ are LCRs used to calculate the noise variance via \eqref{eq:noise_variance}.


\subsubsection{Target $\hat{E}$ Edges}

The last issue is the designation of targeted $\hat{E}$ edges.
$\hat{E}$ should be chosen so that each clique $m$ discovered in KCG $\cG^{(k)}$ has enough nodes to reliably compute mean $\bar{x}_m$ and variance $\sigma_m^2$. 
We estimate $\hat{E}$ as follows.
Given input graph $\cG$, we first compute the average degree $\bar{d}$. 
Then, we target a given clique to have an average of $n_c$ nodes---large enough to reliably compute mean and variance. 
Thus, the average degree of the resulting graph can be approximated as $\bar{d}+n_c-1$. 
Finally, we compute $\hat{E} = \approx N(\bar{d}+n_c-1)$, where $N$ is the number of nodes in the input graph $\cG$.


\subsection{Deriving Weight Parameter} 

\begin{figure}[t]
\centering
\includegraphics[width=0.6\columnwidth]{MSE2.png}
\caption{Bias $B(\mu)$, variance $V(\mu)$, and MSE($\mu$), as functions of weight parameter $\mu$, for a signal with respect to a graph constructed in Section~\ref{sec:graph_learning}. The underlying graph is constructed by connecting adjacent counties in Iowa. 
Graph signal $\x^{o}$ is the clay percentages in each county. 
We assume $\sigma^2=1$ when computing $B(\mu)$, $V(\mu)$, and MSE($\mu$) in \eqref{eq:MSE}.
}
\label{fig:functions}
\end{figure} 

\begin{figure}[t]
\centering
%\hspace{-30pt}
%\vspace{-10pt}
\includegraphics[width=0.235\textwidth]{eig_2}
\label{fig:pcd-on}
%\hspace{-10pt}
\includegraphics[width=0.235\textwidth]{energy_2}
\label{fig:pcd-off}
\caption{(a) Modeling $\lambda_i$'s as an exponentially increasing function $f(i)$; (b) modeling $\alpha_i^2$ as an exponentially decreasing function $g(i)$.} %~\cite{bernardini1999}
\label{fig:approximations}
%\vspace{-14pt}
\end{figure}


Having estimated a noise variance $\sigma^2$, we now derive the optimal weight parameter $\mu$ for MAP formulation \eqref{eq:MAP}.
%Denote by $(\lambda_i,\v_i)$ the $i$-th eigen-pair of graph Laplacian $\L$ corresponding to graph $\cG$. 
Following the derivation in \cite{chen17}, given $\sigma^2$, the mean square error (MSE) of the MAP estimate $\x^*$ from \eqref{eq:MAP} computed using ground truth signal $\x^o$ as function of $\mu$ is
\begin{align}
\text{MSE}(\mu) = \underbrace{\sum_{i=2}^N \psi_i^2 (\v_i^\top \x^o)^2}_{B(\mu)} + \underbrace{\sigma^2 \sum_{i=1}^N \phi_i^2}_{V(\mu)} 
\label{eq:MSE}
\end{align}
where $\psi_i = \frac{1}{1 + \frac{1}{\mu \lambda_i}}$ and $\phi_i = \frac{1}{1 + \mu \lambda_i}$. 
The first term $B(\mu)$ corresponds to the \textit{bias} of estimate $\x^*$, which is a differentiable, \textit{concave} and monotonically increasing function of $\mu>0$.
In contrast, the second term $V(\mu)$ corresponds to the \textit{variance} of $\x^*$, and is a differentiable, \textit{convex} monotonically decreasing function of $\mu>0$. 
\red{discuss previous approach and their convex upper-bound function. show an example of why this is a loose upper bound and thus does not provide a good enough approximation.}

When combined, MSE is a differentiable and provably \textit{pseudo-convex} function of $\mu>0$ \cite{mangasarian1975pseudo}, \ie, 
\begin{align}
\nabla \text{MSE}(\mu_1) \cdot (\mu_2 - \mu_1) \geq 0 \rightarrow \text{MSE}(\mu_2) \geq \text{MSE}(\mu_1),
\label{eq:covex_def}
\end{align}
$\forall \mu_1, \mu_2 >0$.
See Fig.\;\ref{fig:functions} for an example of bias $B(\mu)$, variance $V(\mu)$ and $\text{MSE}(\mu)$ for a specific graph signal $\x^o$ and a graph $\cG$, and Appendix~\ref{app:convex} for a proof of pseudo-convexity. 

In \cite{chen17}, the authors derived a corollary where $\text{MSE}(\mu)$ in \eqref{eq:MSE} is replaced by a convex upper bound $\text{MSE}^+(\mu)$ that is more easily computable.
The optimal $\mu$ is then computed by minimizing the convex function $\text{MSE}^+(\mu)$ using conventional optimization methods. 
However, this upper bound is too loose in practice to be useful.

Instead, we take an alternative approach: we approximate \eqref{eq:MSE} by modeling the distributions of eigenvalues $\lambda_i$'s of $\L$ and signal energies $\alpha_i^2 = (\v_i^\top \x^o)^2$ at graph frequencies $i$ as follows. 
We model $\lambda_i$'s as an exponentially increasing function $f(i)$, and model $\alpha_i^2$ as an exponentially decreasing function $g\left(i\right)$, namely
\red{why these functions? justifications? can we do better?}
\begin{equation}
    \lambda_i\approx f(i)=q\exp\{\gamma i\}; \hspace{10pt} \alpha_i^2\approx g(i)=r\exp\{-\theta i\},
    \label{eq:approx_func}
\end{equation}
where $q, \gamma, r, \theta$ are parameters. 
See Fig.\;\ref{fig:approximations} for illustrations of both approximations.  
To compute those parameters, we first compute extreme eigen-pairs $(\lambda_i, \v_i)$ for $i \in \{2, N\}$ in linear time using LOBPCG~\cite{knyazev2001}. 
Hence we have following expressions from~(\ref{eq:approx_func}),
\begin{equation}
\begin{split}
    \lambda_2 &\approx q\exp\{2\gamma\}; \hspace{20pt} \lambda_N \approx q\exp\{N\gamma\},\\ \alpha_2^2 &\approx r\exp\{-2\theta\}; \hspace{15pt} \alpha_N^2 \approx r\exp\{-N\theta\}. 
\end{split}    
\end{equation}
By solving these equations, one can obtain the four parameters as
\begin{equation}
\begin{split}
    \gamma &= \frac{\ln{\frac{\lambda_N}{\lambda_2}}}{N-2}; \hspace{15pt} q=\lambda_2\exp\left\{-2\frac{\ln{\frac{\lambda_N}{\lambda_2}}}{N-2}\right\},\\
    \theta &= -\frac{\ln{\frac{\alpha_N^2}{\alpha_2^2}}}{N-2}; \hspace{10pt} r=\alpha_2^2\exp\left\{-2\frac{\ln{\frac{\alpha_N^2}{\alpha_2^2}}}{N-2}\right\}.
\end{split}
\end{equation}
One can thus approximate MSE in~(\ref{eq:MSE}) as
\begin{align}
\text{MSE}^a(\mu) = 
\sum_{i=2}^N \frac{g(i)}{\left(1+\frac{1}{\mu f(i)}\right)^2}
+ \sigma^2 \sum_{i=1}^N \frac{1}{\left(1 + \mu f(i)\right)^2} .
\label{eq:approx_MSE}
\end{align}

Since MSE in~(\ref{eq:MSE}) is a differentiable and pseudo-convex function for $\mu >0$, $\text{MSE}^a$ in~(\ref{eq:approx_MSE}) is also a differentiable and pseudo-convex function for $\mu>0$ with its gradient equals to
\begin{equation}
 \nabla \text{MSE}^a(\mu)=\sum_{i=2}^{N}\frac{2\mu g(i)f(i)^2-2f(i)\sigma^2}{(1+\mu f(i))^3}.   
\end{equation}
Finally, the optimal $\mu>0$ is computed by iteratively  minimizing the pseudo-convex function~$\text{MSE}^a(\mu)$ using a standard gradient-decent algorithm:
\begin{equation}
    \mu^{(k)}=\mu^{(k-1)}-t\nabla \text{MSE}^a(\mu^{(k-1)}),
\label{eq:GD}    
\end{equation}
where $t$ is the step size and $\mu^{(k)}$ is the value of $\mu$ at the $k$-th iteration. 
We compute \eqref{eq:GD} iteratively until convergence.  



==> journal/system.tex <==
\subsection{Graph Signal Denoising}

Given noisy observations $\y \in \mathbb{R}^N$, one can formulate a signal restoration problem for signal $\x \in \mathbb{R}^N$ using \textit{graph Laplacian regularizer} (GLR) \cite{pang17}:
\begin{align}
\min_{\x} \|\y - \x\|^2_2 + \mu \x^\top \L \x
\label{eq:MAP}
\end{align}
where $\mu > 0$ is a parameter trading off between the fidelity erm $\|\y - \x\|^2_2$ and GLR $\x^\top \L \x$. 


\subsection{Graph Metric Learning}
\label{sec:graph_learning}

Assuming that each node $i \in \cN$ is endowed with a length-$K$ \textit{feature vector} $\f_i \in \mathbb{R}^K$, one can compute edge weight $w_{i,j}$ connecting nodes $i$ and $j$ in $\cG$ as
\begin{align}
w_{i,j} = \exp \left\{ - (\f_i - \f_j)^\top \M (\f_i - \f_j) \right\}    
\end{align}
where $\M \succeq 0$ is a PSD \textit{metric matrix} that determines the square Mahalanobis distance (feature distance) \\
$d_{i,j} = (\f_i - \f_j)^\top \M (\f_i - \f_j) \geq 0$ between nodes $i$ and $j$. 
There exist \textit{metric learning} schemes \cite{wei_TSP2020,yang21} that optimize $\M$ given an objective function $f(\M)$ and training data $\cX = \{\x_1, \ldots, \x_T\}$. 
For example, we can define $f(\M)$ as
\begin{align}
\min_{\M \succeq 0} f(\M) = \sum_{t=1}^T \x_t^\top \L(\M) \x_t .
\end{align}
In this paper, we adopt an existing metric learning scheme \cite{wei_TSP2020}, and use soil- and location-related features---clay percentage, available water storage estimate (AWS), soil organic carbon stock estimate (SOC) and 2D location features---to compose $\f_i \in \mathbb{R}^5$.
These features are comparatively noise-free and thus reliable.
We use also these features as training data $\cX$ to optimize $\M$, resulting in graph $\cG$. 
(Node pair $(i,j)$ with distance $d_{i,j}$ larger than a threshold has no edge $(i,j) \not\in \cE$). 
We will use $\cG$ to denoise two EVI features that are important for yield prediction.
